Combinatorial slicing problems of polytopes: How (not) to reconstruct a polytope from its slices

We study combinatorial aspects of hyperplane sections of polytopes, focusing on how much the combinatorics of the sections determines the combinatorics of the original polytope. We show that, in general, combinatorial information about the sections is not enough to determine even the $f$-vector of the polytope. In contrast, for sufficiently generic simple polytopes, the function recording the number of vertices of each central section determines the full combinatorial type. We organize different combinatorial slicing properties into hierarchies, separately for affine and central sections, according to the level of combinatorial structure they determine on the polytope. In analogy with classical metric slicing problems, we formulate combinatorial analogues of the Busemann-Petty problem and Bourgain's slicing problem by replacing volume with face numbers, and show that they fail in every dimension and every face dimension.

==> commands.tex <==
%% This is where math commands go %%



\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\sphere}{\mathbb{S}}
\newcommand{\Sph}{\sphere}

\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Hcaltilde}{\widetilde{\Hcal}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Gcal}{\mathcal{G}}

\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bc}{\mathbf{c}}

\newcommand{\cv}[1]{\textsc{#1}}

\newcommand{\case}[1]{\underline{\emph{Case #1:}}}

\DeclareMathOperator{\Bip}{Bip}


\DeclareMathOperator{\OM}{OM}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\cone}{cone}
\DeclareMathOperator{\cl}{cl}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\lin}{lin}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\Vol}{Vol}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\aff}{aff}
\newcommand{\origin}{\mathbf{0}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}
\DeclareMathOperator{\relint}{relint}
\DeclareMathOperator{\inter}{int}
\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\intr}{int}
\DeclareMathOperator{\strip}{strip}
\DeclareMathOperator{\slab}{slab}

\DeclareMathOperator{\verts}{vert}
\DeclareMathOperator{\edges}{edges}
\DeclareMathOperator{\globe}{globe}
\DeclareMathOperator{\base}{base}

\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\ehr}{ehr}
\DeclareMathOperator{\Ehr}{Ehr}
\newcommand{\hstar}{$h^*$}
\DeclareMathOperator{\rk}{rk}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\Real}{Re}
\DeclareMathOperator{\codeg}{codeg}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}

\newcommand{\inner}[1]{ \langle #1 \rangle }
\newcommand{\ma}{\begin{pmatrix}}
\newcommand{\trix}{\end{pmatrix}}
\newcommand{\sma}{\left(\begin{smallmatrix}}
\newcommand{\strix}{\end{smallmatrix}\right)}
\newcommand{\midvert}{\, \Bigg\vert \,}
\newcommand{\scalar}[2]{\langle #1, #2 \rangle}
\newcommand{\norm}[1]{\Vert #1 \Vert}

\newcommand{\thh}{$^{\text{th}}$}

\newcommand{\lp}{\left (}
\newcommand{\rp}{\right )}
\newcommand{\lb}{\left \{}
\newcommand{\rb}{\right \}}

\DeclareMathOperator{\pyr}{pyr}
\DeclareMathOperator{\bipyr}{bipyr}
\DeclareMathOperator{\prism}{prism}

\newcommand{\covers}{\,\cdot\!\!\succ}
\newcommand{\coveredby}{\prec\!\!\cdot\,}



% Widely hacky and unstable commands
\newcommand{\coveredH}{\preceq_{\hspace{1pt}H}$\begin{minipage}{3pt}\vspace*{-1.5pt}$\hspace{-10pt}\cdot$\end{minipage}$}
\newcommand{\coveredP}{\preceq_{\hspace{1pt}P}$\begin{minipage}{3pt}\vspace*{-1.5pt}$\hspace{-9pt}\cdot$\end{minipage}$}

